Non-Rigid Designators in Epistemic and Temporal Free Description Logics (Extended Version)

Definite descriptions, such as 'the smallest planet in the Solar System', have been recently recognised as semantically transparent devices for object identification in knowledge representation formalisms. Along with individual names, they have been introduced also in the context of description logic languages, enriching the expressivity of standard nominal constructors. Moreover, in the first-order modal logic literature, definite descriptions have been widely investigated for their non-rigid behaviour, which allows them to denote different objects at different states. In this direction, we introduce epistemic and temporal extensions of standard description logics, with nominals and the universal role, additionally equipped with definite descriptions constructors. Regarding names and descriptions, in these languages we allow for: possible lack of denotation, ensured by partial models, coming from free logic semantics as a generalisation of the classical ones; and non-rigid designation features, obtained by assigning to terms distinct values across states, as opposed to the standard rigidity condition on individual expressions. In the absence of the rigid designator assumption, we show that the satisfiability problem for epistemic free description logics is NExpTime-complete, while satisfiability for temporal free description logics over linear time structures is undecidable.

==> 0-short-abstract.tex <==
\begin{abstract}
  % Definite descriptions, such as `the smallest planet in the Solar System', have been recently recognised as semantically transparent devices for object identification in knowledge representation formalisms.
Definite descriptions, along with individual names, have been introduced also in the context of description logic languages, enriching the expressivity of standard nominal constructors.
Moreover, in the first-order modal logic literature, definite descriptions have been widely investigated for their \emph{non-rigid} behaviour, which allows them to denote different objects at different states.
%in, e.g., epistemic or  temporal settings.
In this direction, we introduce \emph{epistemic} and \emph{temporal} extensions of standard description logics, with nominals and the universal role, additionally equipped with definite descriptions constructors.
% Regarding names and descriptions, in these languages we allow for: possible \emph{lack of denotation}, ensured by \emph{partial} models, coming from free logic semantics as a generalisation of the classical ones; and \emph{non-rigid designation} features, obtained by assigning to terms distinct values across states, as opposed to the standard rigidity condition on individual expressions.
%from first-order modal logic.
In the absence of the rigid designator assumption, we show that the satisfiability problem for epistemic free description logics is $\NExpTime$-complete, while satisfiability for temporal free description logics
%with non-rigid individual names or definite descriptions
over linear time structures is undecidable.
\end{abstract}


==> CEURART-DL/Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)

%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	# qpdf --linearize --newline-before-endstream $@ /tmp/$@
	# mv /tmp/$@ $@

unminted:
	@./minted2listings "*+minted.tex"

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

